Network Agnostic MPC with Statistical Security

We initiate the study of the network agnostic MPC protocols with statistical security. Network agnostic protocols give the best possible security guarantees irrespective of the underlying network type. We consider the general-adversary model, where the adversary is characterized by an adversary structure which enumerates all possible candidate subsets of corrupt parties. The $\mathcal{Q}^{(k)}$ condition enforces that the union of no $k$ subsets from the adversary structure covers the party set. Given an unconditionally-secure PKI setup, known statistically-secure synchronous MPC protocols are secure against adversary structures satisfying the $\mathcal{Q}^{(2)}$ condition. Known statistically-secure asynchronous MPC protocols can tolerate $\mathcal{Q}^{(3)}$ adversary structures. Fix a set of $n$ parties $\mathcal{P} = \{P_1, ... ,P_n\}$ and adversary structures $\mathcal{Z}_s$ and $\mathcal{Z}_a$, satisfying the $\mathcal{Q}^{(2)}$ and $\mathcal{Q}^{(3)}$ conditions respectively, where $\mathcal{Z}_a \subset \mathcal{Z}_s$. Then, given an unconditionally-secure PKI, we ask whether it is possible to design a statistically-secure MPC protocol resilient against $\mathcal{Z}_s$ and $\mathcal{Z}_a$ in a synchronous and an asynchronous network respectively if the parties in $\mathcal{P}$ are unaware of the network type. We show that it is possible iff $\mathcal{Z}_s$ and $\mathcal{Z}_a$ satisfy the $\mathcal{Q}^{(2,1)}$ condition, meaning that the union of any two subsets from $\mathcal{Z}_s$ and any one subset from $\mathcal{Z}_a$ is a proper subset of $\mathcal{P}$. We design several important network agnostic building blocks with the $\mathcal{Q}^{(2,1)}$ condition, such as Byzantine broadcast, Byzantine agreement, information checking protocol, verifiable secret-sharing and secure multiplication protocol, whose complexity is polynomial in $n$ and $|\mathcal{Z}_s|$.

==> abstractLong.tex <==
In this work, we initiate the study of network agnostic MPC protocols with {\it statistical} security. Network agnostic MPC protocols give the best possible security guarantees to the protocol participants,
 {\it irrespective} of the underlying network type, where the participants are {\it unaware} whether the underlying network is synchronous or asynchronous. While network agnostic MPC
  protocols have been designed earlier for {\it perfect} security and {\it computational} security, to the best of our knowledge, {\it nothing} is known in the literature regarding the possibility of
  network agnostic MPC protocols with statistical security. We consider the {\it general-adversary} model, where the adversary is characterized by an {\it adversary structure}, which enumerates all possible candidate subsets of corrupt parties. Given an unconditionally-secure PKI setup (a.k.a pseudo-signature setup), 
  known statistically-secure {\it synchronous} MPC (SMPC) protocols are secure against adversary structures satisfying the
  $\Q^{(2)}$ condition, meaning that the union of {\it any two} subsets from the adversary structure {\it does not} cover the entire set of parties.
  On the other hand, known statistically-secure {\it asynchronous} MPC (AMPC) protocols 
  can tolerate $\Q^{(3)}$ adversary structures where the union of {\it any three} subsets from the adversary structure {\it does not} cover the entire set of parties.
  
  Fix a set of $n$ parties $\PartySet = \{P_1, \ldots, P_n \}$ and adversary structures $\Z_s$ and $\Z_a$, satisfying the $\Q^{(2)}$ and $\Q^{(3)}$ conditions respectively, where
   $\Z_a \subset \Z_s$.  Then given an unconditionally-secure PKI, we ask whether it is possible to design a statistically-secure MPC protocol, which is resilient against $\Z_s$ in a {\it synchronous}
   network and is resilient against $\Z_a$ in an {\it asynchronous}
   network, even if the parties in $\PartySet$ are unaware of the network type. We show that it is possible if and only if
   $\Z_s$ and $\Z_a$ satisfy the $\Q^{(2, 1)}$ condition, meaning that the union of any two subsets from $\Z_s$ and any one subset from $\Z_a$
   is a proper subset of $\PartySet$. 
     Enroute our MPC protocol, we design several important network agnostic building blocks against general adversaries with the $\Q^{(2, 1)}$ condition, such as Byzantine {\it broadcast},
  {\it Byzantine agreement} (BA), {\it information checking protocol} (ICP), {\it verifiable secret-sharing} (VSS) and secure multiplication protocol.
  The complexity of our building blocks is polynomial in $n$ and $|\Z_s|$.

==> introDetailed.tex <==
\section{Introduction}
\label{sec:intro}
%---
A central concept in modern cryptography is that of secure {\it multiparty computation} (MPC) \cite{Yao82,GMW87,BGW88,RB89}. Informally, an MPC protocol allows a set of $n$ mutually distrusting parties
 $\PartySet = \{P_1, \ldots, P_n \}$ with private inputs, to securely compute any publicly known function $f$ of their inputs, by keeping their respective inputs as private as possible.
  This is achieved even if a subset of the parties are under the control of a centralized {\it adversary} and deviates from the protocol instructions arbitrarily and behaving {\it maliciously} in a Byzantine fashion,  
   during the protocol execution.
   Abstractly, an MPC protocol allows
  the parties in $\PartySet$ to decentralize the role of a virtual {\it trusted third party} (TTP), in the presence of which the parties could perform any secure computation. Due to its powerful abstraction, the MPC problem has
   been widely studied over the last three decades, both by the cryptography as well as distributed computing community and several interesting and fundamental results have been obtained regarding the possibility, 
   feasibility and optimality of MPC in various settings (see for instance \cite{Lin21,CP} and their references).
   
   In any MPC protocol, the parties need to interact by sending messages over the underlying communication network. Two types of networks have been predominantly considered in the literature. 
   The more popular {\it synchronous} MPC (SMPC) protocols operate assuming a synchronous network. Here the participants are assumed to be synchronized and there exists a strict upper bound on message delays
   and every sent message is supposed to be delivered within $\Delta$ time. Consequently, the protocols in this model are executed as a sequence of {\it rounds}, where in each round a party performs some computation,
   computes the messages to be sent to the other parties, sent those messages and finally receive the messages sent to it by the other parties, in that order. In any SMPC protocol, if a receiving party does not receive an expected
   message during a round, then it knows for sure that the corresponding sender party is {\it corrupt} and can accordingly take appropriate ``action", as per the protocol instructions.
   
   Though theoretically appealing, the synchronous model {\it does not} capture the real world networks like the Internet appropriately, where messages can be {\it arbitrarily} delayed. 
   Such networks are better modelled by the {\it asynchronous} communication model with {\it eventual} delivery \cite{CanettiThesis}. In any {\it asynchronous} MPC (AMPC) protocol \cite{BCG93,BKR94}, there are {\it no}
   timing assumptions on message delays and messages can be arbitrarily, yet finitely delayed. The only guarantee is that every sent message will be {\it eventually} delivered. 
   The major challenge in designing protocols in this model is that no participant will known how long it has to wait for an expected message, since a potentially {\it corrupt} sender party (who has {\it not} sent any message)
   {\it cannot} be distinguished from a {\it slow-but-honest} sender party (whose messages are delayed arbitrarily). Consequently, in any AMPC protocol, a party {\it cannot} afford to receive messages from all the $n$ parties,
   to avoid an endless wait, as the potentially corrupt parties may never send their designated messages. Hence, to make ``progress", as soon a party receives messages from a ``subset" of the parties, it has to process them and
   proceed as per the protocol. Unlike the SMPC protocols, AMPC protocols are executed in an event-based fashion, 
      where events are triggered as and when any message is received by a party, which further depends upon the order in which the messages are scheduled for delivery by the underlying network.
      To model the worst case scenario, it is assumed that the scheduling is under the adversary's control. 
   
   Both SMPC and AMPC protocols have their pros and cons. For instance, SMPC protocols are relatively simpler and enjoy better {\it fault-tolerance} (which is the maximum number of faults tolerable) compared to AMPC protocols.
   However, to implement SMPC protocols, one has to pessimistically set the delay $\Delta$, so that the messages of all non-faulty parties are delivered by the end of each round. Consequently, even if a {\it single} message
   (from a non-faulty party) gets delayed beyond $\Delta$ time, then all the security guarantees are at loss. AMPC protocols do not suffer from this shortcoming, since the security {\it does not} depend upon the message delays.
   In fact, any AMPC protocol enjoys the benefit of having a running time, which is proportional to the {\it actual} network delay $\delta$, instead of the round-time delay $\Delta$. 
   On the negative side, AMPC protocols are far more complex than SMPC protocols and enjoy poor fault-tolerance.
    Moreover, every AMPC protocol suffers from what is known as {\it input deprivation} \cite{BH07}, where inputs of {\it all} non-faulty parties
   {\it may not} be considered for the computation of $f$, since waiting for the inputs of all the parties may lead to an endless wait.
   %----
   \paragraph{\bf Network Agnostic MPC Protocols.}
   %--- 
   Apart from SMPC and AMPC protocols, a third category of MPC protocols called network agnostic MPC protocols also exist \cite{} \commentAC{Give references to the network agnostic MPC protocols}.
    In such a protocol, the parties {\it will not} be knowing the exact network type.
    If the network is synchronous then the resultant security guarantees (and fault tolerance) are the same as that of any SMPC protocol.
    On the other hand, if the network is asynchronous, then the resultant security guarantees (and fault tolerance) are the same as that of any AMPC protocol.
    Such protocols are practically motivated, since the protocol participants {\it need not} have to worry about the exact network type
    and the security is maintained, {\it irrespective} of the network type.
    Compare this with a scenario where for example, an SMPC protocol is executed
    {\it assuming} that the network will behave synchronously but instead the network turns out to behave asynchronously (with protocol participants being unaware of this fact),
     thus resulting in the complete security breach. Or it could be the case that the participants execute an AMPC protocol {\it assuming} an asynchronous network, but the network turns out to be
     synchronous (with protocol participants being unaware of this fact), thus resulting in tolerating ``lesser" number of faults than what could have been tolerated by an SMPC protocol.
     %-------
     \subsection{Our Motivation and Results}
     %---
     One of the earliest demarcations made in the literature is to categorize MPC protocols based on the computing power of the underlying adversary. Here, we have two main categories of MPC protocols,
     {\it unconditionally-secure} MPC protocols which remain secure even against  {\it computationally-unbounded} adversaries and
      {\it conditionally-secure} MPC protocols (also called {\it cryptographically-secure}) which remain
     secure only against {\it computationally-bounded} adversaries \cite{Yao82,GMW87}.
     The former category of protocols provide ever-lasting security and are computationally faster than the latter category of protocols, as they are based on relatively simpler operations.
     Unconditionally-secure protocols can be further categorized as {\it perfectly-secure} \cite{BGW88,BCG93} or {\it statistically-secure} \cite{RB89,BKR94};
     while the first category of protocols provide all security guarantees in an {\it error-free} fashion, the second category of protocols achieve the security properties
     except with a {\it negligible} error probability. The fault-tolerance of statistically-secure MPC protocols are significantly {\it better}
      compared to perfectly-secure protocols.
     
     The above demarcation carries over even for network agnostic MPC protocols. While perfectly-secure and cryptographically-secure network agnostic MPC protocols have been investigated earlier \cite{}
     \commentAC{Give references}, to the best of our knowledge, {\it nothing} is known in the literature regarding network agnostic statistically-secure MPC protocols, which is the main motivation of this work.
     In this work we study network agnostic MPC protocols with statistical security for the {\it first} time and derive necessary and sufficient condition for such protocols.
     %----
     \paragraph{\bf Existing Results for Statistically-Secure MPC.}
     %---
     Statistically-secure MPC has been studied earlier, both in the {\it synchronous} as well as in the {\it asynchronous} communication model.
     Consider first the {\it threshold} setting, where the maximum number of corrupt parties under adversary's control is upper bounded by a given threshold. 
     In this model, statistically-secure SMPC tolerating up to $t_s$ faulty parties is possible if and only if $t_s < n/2$ \cite{RB89},
      provided the parties are given some {\it unconditionally-secure} PKI (a.k.a {\it pseudo-signature} setup) \cite{PW96,FitziThesis}.\footnote{The pseudo-signature setup is required to securely realize
      Byzantine agreement (BA) \cite{PeaseJACM80} with $t_s < n/2$.}
      On the other hand, statistically-secure AMPC tolerating up to $t_a$ faulty parties is possible if and only if $t_a < n/3$ \cite{BKR94,ADS20}.
      
      A more generalized form of corruption is modelled through a generalized adversary (also known as the {\it non-threshold} adversarial model), introduced in \cite{HM97}.
      In this model, the corruption capacity of the adversary is captured through a publicly known {\it adversary structure} $\Z \subset 2^{\PartySet}$, which is the set of all subsets of potentially
      corruptible parties and during the protocol execution, adversary is allowed to choose any one subset from $\Z$ for corruption. There are several ``merits" of modelling corruption through an adversary structure, such as:
      %---
      \begin{myitemize}
      %---
      \item[--] It provides more flexibility to model corruption in a fine-grained fashion, compared to the threshold model, where the assumption is that the adversary has the ``resources" to corrupt {\it any} subset of
      given threshold number of parties.
      %---
      \item[--] A threshold adversary is always a ``special" type of non-threshold adversary, where adversary structure $\Z$ has all subsets of $\PartySet$ of size up to $t$, if the underlying threshold is $t$.
      Consequently, a protocol in the non-threshold setting {\it always} imply a protocol in the threshold setting, but the other way around need not be true.
      %---
      \end{myitemize}
      %---
      The downside is that unlike the threshold model, the complexity of the protocols in the non-threshold model is polynomial in $n$ and $|\Z|$, where the latter could be $\Order(2^n)$ in the {\it worst} case.
      In fact, as mentioned in \cite{HM97,HM00}, this is unavoidable. Following the notation of \cite{HM97}, given a subset of parties $\PartySet' \subseteq \PartySet$ and an adversary structure $\Z$, we say that
      $\Z$ satisfies the $\Q^{(k)}(\PartySet', \Z)$ condition, if the union of any $k$ subsets from $\Z$ does not cover $\PartySet'$. That is, the following holds for any subsets $Z_{i_1}, \ldots, Z_{i_k} \in \Z$:
      %----
      \[ (Z_{i_1} \cup \ldots \cup Z_{i_k}) \subset \PartySet'.  \]
       %---  
       In the non-threshold model, it is known that statistically-secure SMPC is possible if and only if the underlying adversary structure $\Z_s$ satisfies the $\Q^{(2)}(\PartySet, \Z_s)$ condition, provided the parties are
       given an unconditionally-secure PKI setup \cite{HT13}, while statistically-secure AMPC requires the underlying adversary structure $\Z_a$ to satisfy the $\Q^{(3)}(\PartySet, \Z_a)$ condition \cite{HT13,ACC22c}.
       %-----
       \paragraph{\bf Our Results for Network Agnostic Statistically-Secure MPC.}
       %---
       In this work, we study the possibility of network agnostic MPC protocol with statistical security. We consider the most generic form of corruption, namely the non-threshold adversary model. 
       We ask the following question:
       %---
       \begin{center}
       %---
       Given an unconditionally-secure PKI, a {\it synchronous adversary structure} $\Z_s$ and an {\it asynchronous adversary structure} $\Z_a$, satisfying the 
       $\Q^{(2)}(\PartySet, \Z_s)$  and  $\Q^{(3)}(\PartySet, \Z_a)$ conditions respectively where $\Z_a \subset \Z_s$, does there exist a statistically-secure MPC protocol, which remains secure against
       $\Z_s$ and $\Z_a$ in a synchronous and asynchronous network respectively?      
       %---
       \end{center}
       %----
       We answer the above question affirmatively, if and only if $\Z_s$ and $\Z_a$ satisfy the $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition, meaning that for any $Z_{i_1}, Z_{i_2} \in \Z_s$ and ${\mathsf Z}_{j} \in \Z_a$, the following
       holds:
       %---
       \[ (Z_{i_1} \cup Z_{i_2} \cup {\mathsf Z}_j) \subset \PartySet.\]
       %---
       In general, we say that $\Z_s$ and $\Z_a$ satisfy the $\Q^{(k, k')}(\PartySet, \Z_s, \Z_a)$ condition, if for any $Z_{i_1}, \ldots, Z_{i_k} \in \Z_s$ and ${\mathsf Z}_{j_1}, \ldots, {\mathsf Z}_{j_{k'}} \in \Z_a$, the following
       holds:
       %---
       \[ (Z_{i_1} \cup \ldots \cup Z_{i_k} \cup {\mathsf Z}_{j_1} \cup \ldots \cup {\mathsf Z}_{j_k'}) \subset \PartySet.\]
       %---
       To show the sufficiency of the $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ 
        condition, we present a network agnostic statistically-secure MPC protocol with the same condition, whose complexity is polynomial in $n$ and $|\Z_s|$.
       Our results when applied against {\it threshold} adversaries imply that given an unconditionally-secure PKI, and thresholds $0 < t_a <  \frac{n}{3} < t_s < n/2$, network agnostic
        statistically-secure MPC tolerating $t_s$ and $t_a$ corruptions in the {\it synchronous} and {\it asynchronous} network is 
        possible, if and only if $2t_s + t_a < n$ holds. The complexity of the resultant protocol is polynomial in $n$ and ${n \choose t_s}$. Our results in the context of relevant literature is summarized in 
        Table \ref{tab:Summary}.
        %----    
             \begin{table}[!htb]
         	\begin{center}
	\begin{adjustbox}{width=1\textwidth}
			\begin{tabular}{|c|c|c|c|c|}
			\hline
			%---
			Network Type & Corruption Scenario & Security & Condition & Reference \\ \hline
			%---
			Synchronous & Threshold $(t)$ & Perfect & $t < n/3$ & \cite{BGW88} \\ \hline
			%--
			Synchronous & Non-threshold $(\Z)$ & Perfect & $\Q^{(3)}(\PartySet, \Z)$ & \cite{HM97} \\ \hline
			%--
			Synchronous & Threshold $(t)$ & Statistical & $t < n/2$ & \cite{RB89} \\ \hline
			%--	
			Synchronous & Non-threshold $(\Z)$ & Statistical & $\Q^{(2)}(\PartySet, \Z)$ & \cite{HT13} \\ \hline \hline
			%--
			Asynchronous & Threshold $(t)$ & Perfect & $t < n/4$ & \cite{BCG93} \\ \hline
			%--
			Asynchronous & Non-threshold $(\Z)$ & Perfect & $\Q^{(4)}(\PartySet, \Z)$ & \cite{MSR02} \\ \hline
			%--
			Asynchronous & Threshold $(t)$ & Statistical & $t < n/3$ & \cite{BKR94,ADS20} \\ \hline
			%--		
			Asynchronous & Non-threshold $(\Z)$ & Statistical & $\Q^{(3)}(\PartySet, \Z)$ & \cite{ACC22c} \\ \hline \hline
			%--
			Network Agnostic & Threshold $(t_s, t_a)$ & Perfect & $0 < t_a < n/4 < t_s < n/3$ & \cite{ACC22a}\\ 
			                             &                                     & &  and $3t_s + t_a < n$         &       \\ \hline
                         %---			                             
                         Network Agnostic & Non-threshold $(\Z_s, \Z_a)$ & Perfect & $\Z_a \subset \Z_s, \Q^{(3)}(\PartySet, \Z_s), \Q^{(4)}(\PartySet, \Z_a)$ & \cite{ACC22b} \\ 
			                             &                                     & &  and $\Q^{(3, 1)}(\PartySet, \Z_s, \Z_a)$         &       \\ \hline
                         %-----			                             
                         Network Agnostic & Threshold $(t_s, t_a)$ & Computational & $0 < t_a < n/3 < t_s < n/2$ & \cite{BZL20}\\ 
			                             &                                     & &  and $2t_s + t_a < n$         &       \\ \hline \hline
			%---                              
 			 %-----			                             
                          Network Agnostic & Non-threshold $(\Z_s, \Z_a)$ & Statistical & $\Z_a \subset \Z_s, \Q^{(2)}(\PartySet, \Z_s), \Q^{(3)}(\PartySet, \Z_a)$ & This work\\ 
			                             &                                     & &  and $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$         &       \\ \hline          
			  %---                                             
                             Network Agnostic & Threshold $(t_s, t_a)$ & Statistical & $0 < t_a < n/3 < t_s < n/2$ & This work\\ 
			                             &                                     & &  and $2t_s + t_a < n$         &       \\ \hline
						
				\end{tabular}
       \end{adjustbox}				
	\end{center}
	\caption{\label{tab:Summary}Various conditions for MPC in different settings}
	\end{table}
   %-------
 \subsection{Detailed Technical Overview}
 %----
  We follow the standard idea of shared {\it circuit-evaluation} \cite{BGW88,RB89},
   where the function $f$ to be securely computed  is abstracted as a publicly known circuit $\ckt$ over some finite field $\F$ and the goal is to securely evaluate each gate
   in $\ckt$ in a {\it secret-shared} fashion, where for every value during the circuit-evaluation, each party holds a share, such that the shares of the corrupt parties {\it does not} reveal anything additional about the underlying
   value. And once the function output is ready in a secret-shared fashion, it is publicly reconstructed. Intuitively, the security follows since during the circuit-evaluation, the adversary {\it does not} reveal anything additional, beyond
    what it can infer from the inputs of the corrupt parties and the function output, as the shares of the corrupt parties will not reveal anything additional.
    The secret-sharing to be deployed is preferably {\it linear}, which enables the parties to evaluate linear gates in $\ckt$ in a {\it non-interactive} fashion, while {\it non-linear} gates are evaluated using
    the Beaver's method \cite{Bea91}, by deploying secret-shared random {\it multiplication-triples}, which are generated {\it beforehand}. 
    
    The above approach is the defacto and used in all existing {\it unconditionally-secure} protocols, both with perfect as well as statistical security.
     To realize it with {\it statistical} security, we need the following ingredients:
     a {\it Byzantine agreement} (BA) protocol \cite{PeaseJACM80} which allows the parties with different inputs
     to reach agreement on a common value, 
      an {\it information checking protocol} (ICP) \cite{RB89} for authenticating data in a privacy-preserving fashion and with unconditional security,
     a {\it verifiable secret sharing} (VSS) protocol \cite{CGMA85} for verifiably sharing secrets consistently even in the presence of malicious corruptions,
     a {\it reconstruction} protocol for robustly reconstructing secret-shared values and finally a secure {\it multiplication} protocol to securely multiply two secret-shared values.
     All existing statistically-secure SMPC \cite{RB89,CDDHR99,BH06,GSZ20,HT13} and AMPC \cite{BKR94,PCR15,CP17,CP23,ACC22c} protocols have various instantiations of the above building blocks,
     {\it either} in the synchronous {\it or} asynchronous setting, where the parties will be {\it already knowing} the network type.
     However, in our context where the parties will {\it not} be knowing the exact network type, we face several challenges to get instantiation of the above building blocks, which are network agnostic.
     We now take the reader through a detailed tour of the technical challenges and how we deal with them for each of the building blocks and refer to the respective sections for the complete formal details.
     %----
     \subsubsection{Network Agnostic Byzantine Agreement (BA)}
     %---
     In a BA protocol \cite{PeaseJACM80}, each party participates with a private input bit. The protocol allows the parties to agree on a common output bit ({\it consistency}), where the output bit is the input of the
     non-faulty parties, if all of them have the same input bit ({\it validity}).
     Given an unconditionally-secure PKI, {\it synchronous} BA (SBA) is possible if and only if the underlying adversary structure $\Z_s$ satisfies the $\Q^{(2)}(\PartySet, \Z_s)$ condition \cite{PW96,FM98,FitziThesis}, while
     {\it asynchronous} BA (ABA) requires the underlying adversary structure $\Z_a$ to satisfy the $\Q^{(3)}(\PartySet, \Z_s)$ condition \cite{Cho23}.
     Existing SBA protocols become completely {\it insecure} when executed in an asynchronous network, if even a single messages from a non-faulty party is delayed. 
     On the other hand, any ABA protocol when executed in a synchronous network will {\it satisfy} the validity and consistency properties, provided the underlying adversary structure
     satisfies {\it only} $\Q^{(3)}$ condition, which {\it need not} be the case. Moreover, the {\it liveness} guarantees for SBA and ABA are {\it different}. 
        Namely, SBA requires {\it guaranteed liveness}, meaning that the non-faulty parties get some output after a ``fixed" time. On the other hand, to circumvent the FLP impossibility result \cite{FLP85}, ABA protocols are
     randomized and provide {\it almost-surely liveness}, where the non-faulty
      parties eventually get an output, asymptotically with probability $1$. That is, it is possible that the non-faulty parties keep running the protocol forever without any output, though the probability of this happening
      is $0$. 
      
      To circumvent the above problems, we design a network agnostic BA protocol, provided $\Z_s$ and $\Z_a$ satisfy the $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition. 
      The protocol is obtained by generalizing the blueprint for network agnostic BA, first proposed in \cite{BKL19} and later used in \cite{ACC22a}.
      Both \cite{BKL19} and \cite{ACC22a} proposed the blueprint for {\it threshold} adversaries; while \cite{BKL19} proposed it for {\it computational security}
      with conditions $0 < t_a < n/3 < t_s < n/2$ and $2t_s + t_a < n$ provided the parties are provided a {\it computationally-secure} PKI, later
      \cite{ACC22a} modified it for {\it perfect security}
            and used it with conditions $t_a, t_s < n/3$.\footnote{{\it Unlike} computationally-secure BA, the necessary condition for perfectly-secure BA is $t < n/3$ for {\it both} SBA as well as ABA, where $t$ is
            the maximum number of faults.} We replace the computationally-secure PKI with an {\it unconditionally-secure} PKI and generalize the building blocks of \cite{BKL19} against non-threshold adversaries with
            $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition and upgrade their security to unconditional-security. 
            Additionally, we also generalize certain unconditionally-secure
            primitives from \cite{ACC22a} and adapt them to work with the $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition.
            Then by carefully stitching together these unconditionally-secure building blocks, we get our network agnostic BA protocol.
            Since this part mostly follows the existing protocols, we refer the readers to Section \ref{sec:BA} for full details.
%----------            
     \subsubsection{Network Agnostic ICP with $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ Condition}
     \label{ssec:ICP}
     %---
     An ICP \cite{RB89,CDDHR99} is used for authenticating data in the presence of a 
  {\it computationally-unbounded} adversary. 
  In an ICP, there are {\it four} entities, a {\it signer} $\mathsf{S} \in \PartySet$,
   an  {\it intermediary} $\mathsf{I} \in \PartySet$, a {\it receiver}
  $\mathsf{R} \in \PartySet$ and all the parties in $\PartySet$ acting as {\it verifiers}
   (note that $\mathsf{S}, \mathsf{I}$ and $\mathsf{R}$ also act as verifiers).
    An ICP has two sub-protocols, one for the {\it authentication phase} and one for 
    the {\it revelation phase}. 
    
    In the authentication phase, $\mathsf{S}$ has a private input
    $s \in \F$, which it distributes to $\mathsf{I}$ along with some {\it authentication information}.
    Each verifier is provided with some {\it verification information}, followed by the parties verifying whether $\mathsf{S}$ has distributed ``consistent" information. 
    If the verification is ``successful", then the 
    data held by $\mathsf{I}$ at the end of this phase is called  {\it $\mathsf{S}$'s IC-Signature on $s$ for intermediary $\mathsf{I}$ and receiver $\mathsf{R}$}, denoted by
    $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s)$. 
    Later, during the revelation phase, $\mathsf{I}$ reveals $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s)$ to $\mathsf{R}$,
    who ``verifies" it with respect to the verification information provided by the verifiers and either accepts or rejects
    $s$. We require the same security guarantees from ICP as expected from cryptographic signatures,
    namely {\it correctness} (if $\mathsf{S, I}$ and $\mathsf{R}$ are {\it all} honest, then $\mathsf{R}$ should accept $s$), {\it unforgeability} 
    (a {\it corrupt} $\mathsf{I}$ should fail to reveal an {\it honest} $\mathsf{S}$'s signature on $s' \neq s$) and {\it non-repudiation}
     (if an {\it honest} $\mathsf{I}$ holds some $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s)$, then later an {\it honest} $\mathsf{R}$ should accept
     $s$, even if $\mathsf{S}$ is {\it corrupt}).
       Additionally, we need {\it privacy}, guaranteeing that if 
    $\mathsf{S, I}$ and $\mathsf{R}$ are {\it all} honest, then $\Adv$ does not learn 
    $s$.\footnote{IC-signatures are {\it different} from pseudo-signatures.
    Pseudo-signatures are ``transferable", where a party can transfer a signed message to other parties for verification (depending upon the allowed level
    of transferability), while IC-signatures {\it can} be verified only by the designated $\mathsf{R}$ and {\it cannot} be further transferred. 
    Due to the same reason, IC-signatures satisfy the privacy property unlike pseudo-signatures. Most importantly, IC-signatures are generated from the scratch, assuming a pseudo-signature
    setup which is used to instantiate the instances of broadcast in the ICP.}
    
    Known instantiation of ICP in the {\it synchronous} network \cite{HT13} is secure against $\Q^{(2)}$ adversary structures and become {\it insecure}
    in the {\it asynchronous} setting. On the other hand, known instantiation of ICP in the {\it asynchronous} setting \cite{ACC22c} can tolerate {\it only}
    $\Q^{(3)}$ adversary structures. Our instantiation of network agnostic
     ICP is a careful adaptation of the {\it asynchronous} ICP of \cite{ACC22c}.
     We first try to {\it naively} adapt the ICP to deal with the {\it network agnostic} setting, followed by the technical problems in the naive adaptation
     and the modifications needed.
     
    During the authentication phase, $\mathsf{S}$ embeds $s$ in a random $t$-degree {\it signing-polynomial} $F(x)$ at $x = 0$, where 
    $t$ is the cardinality of maximum-sized subset in $\Z_s$, and gives $F(x)$ to $\mathsf{I}$. In addition, each verifier $P_i$ is given a random {\it verification-point}
    $(\alpha_i, v_i)$ on $F(x)$. 
    To let the parties securely verify that it has distributed consistent information, $\mathsf{S}$
    additionally distributes a random $t$-degree {\it masking-polynomial} $M(x)$ to $\mathsf{I}$, while
    each verifier $P_i$ is given a point on $M(x)$ at $\alpha_i$. Each verifier upon receiving 
    its verification-points, {\it publicly} confirms the same. 
    Upon receiving these confirmation, $\mathsf{I}$ identifies a
    a subset of {\it supporting verifiers} $\R$ who have {\it publicly} confirmed the receipt of their verification-points.
    Since in a {\it synchronous} network, a subset of {\it corrupt} parties from $\Z_s$ {\it may not} respond and
     the  parties {\it will not} know the network type, the parties {\it cannot} afford for {\it all} the verifiers to confirm the receipt of their verification-points, to avoid an endless wait.
    Hence $\mathsf{I}$ waits till 
    $\PartySet \setminus \R \in \Z_s$ holds, after which the parties {\it publicly} check the consistency of the $F(x), M(x)$ polynomials
    and the distributed points, with respect to a {\it random} linear combination of these polynomials and points, where the linear combiner is selected by
     $\mathsf{I}$, once the set $\R$ is decided.
    This ensures that $\mathsf{S}$ has no knowledge beforehand about the random combiner while distributing the points to
    $\R$ and hence, any inconsistency among the data distributed to $\mathsf{I}$ and the verifiers in $\R$ will be detected.
      If no inconsistency is detected, the parties proceed to the revelation phase, where 
    $\mathsf{I}$ reveals $F(x)$ to $\mathsf{R}$, while each verifier in $\R$
    reveals its verification-point to $\mathsf{R}$, who accepts $F(x)$ (and hence $F(0)$), if it
    sure that there exists at least one {\it non-faulty} verifier in $\R$, whose verification point is ``consistent" with the revealed $F(x)$. 
    This would ensure that the revealed $F(x)$ is indeed correct with a high probability, since a potentially {\it corrupt} $\mathsf{I}$ will have no information about the verification point of any
    {\it non-faulty} verifier in $\R$, provided $\S$ is {\it non-faulty}. 
    Since in a {\it synchronous} network, a subset of {\it corrupt} verifiers from $\Z_s$ belonging to $\R$ {\it may not} respond and
     the  parties {\it will not} know the network type, $\mathsf{R}$ {\it cannot} afford for the verification-points of {\it all} the
       verifiers in $\R$, to avoid an endless wait. Hence, as soon as it finds a subset of verifiers $\R' \subseteq \R$, where
      $\R \setminus \R' \in \Z_s$ whose verification-points are found to be consistent with $F(x)$, it outputs $F(0)$.
%-------
   \paragraph{\bf A Technical Problem and Way-out.}
   %---       
   The protocol outlined above will achieve all the required properties in an {\it asynchronous} network,
   This is because the asynchronous ICP of \cite{ACC22c} can tolerate $\Q^{(3)}$ adversary structures and $\Z_a$ in our case indeed satisfies the
   $\Q^{(3)}(\PartySet, \Z_a)$ condition. Moreover, $\Z_a \subset \Z_s$ also holds in our case.
   However, the protocol {\it fails} to satisfy the 
   {\it unforgeability} property in a {\it synchronous} network. Namely, a {\it corrupt} 
   $\mathsf{I}$ may {\it not} include {\it all} the non-faulty verifiers in $\R$ and purposely {\it exclude} a subset of {\it non-faulty} verifiers belonging to $\Z_s$
    (even if these verifiers have publicly confirmed the receipt of their verification points).
   Let $\Hon_{\R}$ be the set of {\it non-faulty} verifiers in $\Hon$ and let $\C_{\R}$ be the set of {\it corrupt} verifiers in $\R$. Due to the above strategy of a corrupt $\mathsf{I}$, 
   the condition $\Q^{(1)}(\Hon_\R, \Z_s)$ {\it may not} be satisfied and $\R \setminus \C_\R = \Hon_\R \in \Z_s$ {\it may hold}.
   As a result, during the revelation phase, $\mathsf{I}$ may produce an {\it incorrect} $F'(x) \neq F(x)$ and the verifiers in $\C_{\R}$ may change their verification points to 
    ``match" $F'(x)$, 
   while only the verification points of the verifiers in $\Hon_\R$ may turn out to be inconsistent with $F'(x)$. Consequently, $\R' = \C_\R$
   and if $\Hon_\R \in \Z_s$, then clearly $F'(x)$ and hence $s' = F'(0)$ will be the output
   of the revelation phase, thus breaking the
   unforgeability property.
   
   To deal with the above issue, {\it instead} of $\mathsf{I}$ selecting $\R$, we let $\S$ to identify and publicly announce the set $\R$. This will ensure that {\it all}
    honest verifiers are present in $\R$, if $\S$ is {\it honest} and the network is {\it synchronous}, provided $\S$ waits for ``sufficient" time to let the verifiers announce the receipt of their verification points.
    Consequently, {\it now} the condition $\Q^{(1)}(\Hon_\R, \Z_s)$ {\it will be} satisfied.
    Hence, if during the revelation phase, a {\it corrupt} $\mathsf{I}$ reveals an incorrect $F'(x) \neq F(x)$, then it will be rejected,
    as the condition $\R \setminus \C_\R \in \Z_s$ {\it no} longer holds. 
   %--- 
      \paragraph{\bf Linearity of ICP.} 
    %---        
 Our ICP satisfies the {\it linearity} property (which will be useful later in our VSS),
  provided ``special care" is taken while generating the IC-signatures. In more detail, 
 consider a {\it fixed} $\mathsf{S}, \mathsf{I}$ and $\mathsf{R}$ and let $s_a$ and $s_b$ be two values, such that $\mathsf{I}$ holds $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s_a)$ and 
  $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s_b)$, where {\it all} the following conditions are satisfied during the underlying instances of the authentication phase.
  %----
  \begin{myitemize}
  %-----
  \item[--] The set of supporting verifiers $\R$ are the {\it same} during both the instances.
  %---
  \item[--] For $i = 1, \ldots, n$, corresponding to the verifier $P_i$, $\mathsf{S}$ has used the {\it same} $\alpha_i$, to compute the verification points, during 
   both the instances.
  %----
  \item[--] $\mathsf{I}$ has used the {\it same} linear combiner to verify the consistency of the distributed data in both the instances.
  %---
  \end{myitemize}
  %-----
  Let $s \defined c_1 \cdot s_a + c_2 \cdot s_b$, where $c_1, c_2$ are {\it publicly known} constants from $\F$. It then follows that if all the above conditions are satisfied, then $\INT$
  can {\it locally} compute $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s)$ from $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s_a)$ and $\ICSig(\mathsf{S}, \mathsf{I}, \mathsf{R}, s_b)$,
   while each verifier in $\R$ can {\it locally} compute their corresponding verification information. 
    %------ 
     \subsubsection{Network Agnostic VSS and Reconstruction}
     \label{ssec:VSS}
     %---
     Since in the network agnostic setting, parties will {\it not} be knowing the network type, to ensure privacy, 
      all the values during the circuit evaluation need to remain private in the ``worst" possible scenario, when 
      the adversary corrupts a subset
     of parties from $\Z_s$. Consequently, all the values are secret-shared ``with respect" to $\Z_s$.
     We follow the notion of {\it additive secret-sharing}, introduced in \cite{ISN87} and also used in the earlier MPC protocols against non-threshold adversaries \cite{Mau02,HT13,ACC22c}.
     Given the adversary structure $\Z_s = \{Z_1, \ldots, Z_{|\Z_s|} \}$, we consider the {\it sharing specification} $\ShareSpec_{\Z_s} = \{S_1, \ldots, S_{|\Z_s|} \}$, where each $S_q = \PartySet \setminus Z_q$. 
     It follows that there exists at least one subset $S_q \in \ShareSpec_{|\Z_s|}$ which {\it does not} contain any faulty party, {\it irrespective} of the network type; while this is trivially true for the {\it synchronous}
     network, it also holds in the {\it asynchronous} network, since $\Z_a \subset \Z_s$.
     A value $s \in \F$ is said to be secret-shared, if there exists shares $s_1, \ldots, s_{|\Z_s|}$ which sum up to $s$, such that all (non-faulty) parties in $S_q$ have the share $s_q$.
     We denote a secret-sharing of $s$ by $[s]$, with $[s]_q$ denoting the share corresponding to the set $S_q$. Note that if the shares $[s]_1, \ldots, [s]_{|\Z_s|}$ are randomly chosen, then the probability
     distribution of the shares learnt by the adversary will be independent of $s$, since at least one share among $[s]_1, \ldots, [s]_{|\Z_s|}$ will be {\it missing} for the adversary.
     We also note that the above secret-sharing is {\it linear}, since given secret-sharings $[a]$ and $[b]$ and publicly known constants $c_1, c_2 \in \F$, the following holds:
     %---
     \[ c_1 \cdot [a] + c_2 \cdot [b] = [c_1 \cdot a + c_2 \cdot b].\]
     %---
     Consequently, the parties can {\it non-interactively} compute any publicly known linear function of secret-shared values. Unfortunately, the above secret-sharing {\it does not} allow for the
     robust reconstruction of a secret-shared value. This is because the corrupt parties may produce {\it incorrect} shares, which are ``indistinguishable" from the shares produced by non-faulty parties. 
     To deal with this, we ``augment" the above secret-sharing, where as part of a secret-sharing of $s$,
     apart from the shares $[s]_1, \ldots, [s]_{|\Z_s|}$, we also have publicly known {\it core-sets}
     $\W_1, \ldots, \W_{|\Z_s|}$, where each $W_q \subseteq S_q$ with $S_q \setminus W_q \in \Z_a$ and where each (non-faulty) $P_i \in \W_q$ will have the IC-signature 
     $\ICSig(P_j, P_i, P_k, [s]_q)$ corresponding to every $P_j \in \W_q$ and every $P_k \not \in \W_q$, such that the underlying IC-signatures satisfy the {\it linearity} property. 
     
     We call the augmented secret sharing as {\it linear secret-sharing with IC-signatures}, which is still denoted as $[s]$. Notice that since $S_q \setminus W_q \in \Z_a$, due to the
     $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition, $\W_q$ is bound to have at least one {\it non-faulty} party, {\it irrespective} of the network type, since $\W_q$ satisfies the
     $\Q^{(1)}(\PartySet, \Z_s)$ condition. To reconstruct $s$ which is linearly secret-shared with IC-signatures, we ask the parties in $\W_q$ to make public the share $[s]_q$. 
     To identify the correct shares, we actually ask each $P_i \in \W_q$ to reveal $\ICSig(P_j, P_i, P_k, [s]_q)$ to $P_k$, corresponding to {\it all} $P_j \in \W_q$.
     Party $P_k$ can then verify whether $[s]_q$ revealed by $P_i$ is {\it correct} by checking if $P_i$ has revealed the correct IC-signature of {\it every} $P_j \in \W_q$ on $[s]_q$.
     If $P_i$ is {\it corrupt} then due to the {\it unforgeability} if ICP, it will fail to forge IC-signature of a {\it non-faulty} $P_j$ on an {\it incorrect} $[s]_q$.
     However, if $P_i$ is {\it non-faulty}, then it will reveal the correct $[s]_q$ and the signature of {\it every} $P_j \in \W_q$ on $[s]_q$, which are accepted even if
     $P_j$ is {\it corrupt} (follows from {\it non-repudiation} of ICP).  
     
     To generate a linear secret-sharing with IC-signature, we design a network agnostic VSS protocol $\VSS$, which allows a designated {\it dealer} $\D \in \PartySet$ with input $s \in \F$, to {\it verifiably} generate
     $[s]$. If $\D$ is {\it non-faulty}, then the parties output $[s]$ after a ``fixed" time in a {\it synchronous} network, and {\it eventually} in an {\it asynchronous} network, with the view of the adversary remaining
     independent of $s$. On the other hand, if $\D$ is {\it faulty} then either no non-faulty party obtains any output (if $\D$ {\it does not} invoke the protocol) or there exists {\it some} $s^{\star} \in \F$, such that the parties
     output $[s^{\star}]$. Note that in the latter case, we {\it cannot} upper bound the time within which the non-faulty parties will output $[s^{\star}]$ {\it even} in a {\it synchronous} network, since a {\it corrupt}
     $\D$ may delay sending the messages and the parties will {\it not} be knowing the network type. To design $\VSS$, we use certain ideas from the statistically-secure
     {\it synchronous} VSS (SVSS) and {\it asynchronous} VSS (AVSS)
     of \cite{HT13} and \cite{ACC22c} respectively, along with some new counter-intuitive ideas. In the sequel, we first give a brief outline of the SVSS and AVSS of \cite{HT13,ACC22c}, followed by the technical challenges
     arising in the network agnostic setting and how we deal with them.
     %-----
     \paragraph{\bf Statistically-Secure SVSS of \cite{HT13} for $\Z_s$ with $\Q^{(2)}(\PartySet, \Z_s)$ Condition.}
     %---
     Let  $\Z_s = \{Z_1, \ldots, Z_{|\Z_s|} \}$ and $\ShareSpec_{\Z_s} = \{S_1, \ldots, S_{|\Z_s|} \}$, where each $S_q = \PartySet \setminus Z_q$.     
     The SVSS of \cite{HT13} 
     proceeds as a sequence of {\it synchronized} phases. During the {\it first} phase, $\D$ picks random shares $s_1, \ldots, s_{|\Z_s|}$ which sum up to $s$ and sends $s_q$ to all the parties in $S_q$.
     To verify whether $\D$ has distributed the same share to all the parties in $S_q$, during the {\it second} phase,
      every pair of parties $P_i, P_j \in S_q$ exchange their supposedly common shares received from $\D$,
      along with their respective IC-signatures. That is $P_i$ upon receiving $s_{qi}$ from $\D$ gives $\{\ICSig(P_i, P_j, P_k, s_{qi})\}_{P_k \in \PartySet}$ to $P_j$, while
      $P_j$ upon receiving $s_{qj}$ from $\D$ gives $\{\ICSig(P_j, P_i, P_k, s_{qi})\}_{P_k \in \PartySet}$ to $P_i$.
      Then during the {\it third} phase, the parties in $S_q$ {\it publicly} complaint about any ``discrepancy" in their supposedly common share, in response to which $\D$ is supposed to make {\it public} the share
      $s_q$ corresponding to $S_q$ during the {\it fourth} phase.
       Hence by the end of {\it fourth} phase it is ensured that for every $S_q \in \ShareSpec_{|\Z_s|}$, either the share $s_q$ is {\it publicly} known (if any complaint was reported for $S_q$)
       or all (non-faulty) parties in $S_q$ have the same share (along with the respective IC-signatures of each other on it).
       Note that the privacy of $s$ is maintained for a {\it non-faulty} $\D$, since the share $s_q$ corresponding to the $S_q$ consisting of {\it only non-faulty} parties  is {\it never} made public.
     %----       
      \paragraph{\bf Statistically-Secure AVSS of \cite{ACC22c} for $\Z_a$ with $\Q^{(3)}(\PartySet, \Z_a)$ Condition.}
     %---
     Let  $\Z_a = \{\mathsf{Z}_1, \ldots, \mathsf{Z}_{|\Z_a|} \}$ and $\ShareSpec_{\Z_a} = \{\S_1, \ldots, \S_{|\Z_a|} \}$, where each $\S_q = \PartySet \setminus \mathsf{Z}_q$.     
     The AVSS protocol of \cite{ACC22c} also follows a similar idea as the SVSS of \cite{HT13}. Namely, $\D$ distributes shares to the parties in each group $\S_q$, followed by the parties in $\S_q$
     exchanging IC-signed versions of their supposedly common share. However, since the network is now {\it asynchronous}, the parties {\it cannot} afford to wait for {\it all} the parties in $\S_q$ to report
     the status of pairwise consistency tests, as the corrupt parties in $\S_q$ may {\it never} turn up. Due to the same reason, even if any complaint is reported for $\S_q$, the parties don't know how long to wait for
     $\D$ to ``resolve" the complaint. Hence {\it instead} of looking for {\it inconsistencies} in $\S_q$, the parties {\it rather} check how many parties in $\S_q$ are reporting for the {\it pairwise consistency} of their supposedly
     common share. The idea is that if $\D$ has distributed shares consistently, then from each $\S_q$, a subset of parties $\W_q$ where $\S_q \setminus \W_q \in \Z_a$ should eventually confirm the receipt of a common share
     from $\D$. Based on this observation, the parties check if there exists subsets of {\it core-parties} $\W_1, \ldots, \W_{|\Z_a|}$, where each $\S_q \setminus \W_q \in \Z_a$, such that the parties
     in $\W_q$ have confirmed the receipt of a common share from $\D$. To ensure that all the parties have agreement on the sets $\W_1, \ldots, \W_{|\Z_a|}$, the dealer is designated the task of
     finding and making public these sets. And the parties proceed further only upon receiving and verifying the existence of these sets. While a {\it non-faulty} $\D$ will eventually find and make public such sets,
     if the existence of such sets is confirmed for a {\it corrupt} $\D$, then it implies that it has committed a common share to all the {\it non-faulty} parties in $\W_q$.
     Note that {\it irrespective} of $\D$, each $\W_q$ is bound to have {\it at least} one non-faulty party, since $\Z_a$ will satisfy the $\Q^{(1)}(\W_q, \Z_a)$ condition.
     
     The existence of $\W_1, \ldots, \W_{|\Z_a|}$ {\it does not} imply that {\it all} non-faulty parties in $\S_q$ have received a common share, even if $\D$ is {\it non-faulty}, since there {\it might} be
     non-faulty parties outside $\W_q$. Hence, 
     after the confirmation and verification of the sets $\W_1, \ldots, \W_{|\Z_a|}$, the goal is to ensure that every (non-faulty) party in $\S_q$, who are ``outside" $\W_q$ (i.e, the parties in $\S_q \setminus \W_q$),
     also get the common share held by the (non-faulty) parties in $\W_q$. For this, 
     the parties in $\W_q$ reveal their shares to these outsider parties, along with the IC-signatures of {\it all} the parties in $\W_q$ on the revealed shares.
     The outsider parties then ``filter" out the correctly revealed shares. 
     The existence of at least one non-faulty party in each $\W_q$ guarantees that the shares filtered by the outsider parties are indeed correct (with a high probability).     
     %---
     \paragraph{\bf Technical Challenges for Network Agnostic VSS and Way Out.}       
     %---
     Since in our context, the parties will {\it not} be knowing the network type, our approach will be to follow the AVSS of \cite{ACC22c}, where we look for {\it pairwise consistencies} of supposedly common share in each group.
     Namely, $\D$ on having the input $s$, picks random shares $s_1, \ldots, s_{|\Z_s|}$ which sum up to $s$ and distributes $s_q$ to each $S_q \in \ShareSpec_{|\Z_s|}$.\footnote{Recall that we want to generate
     $[s]$ with respect to $\Z_s$, {\it irrespective} of the network.}. The parties in $S_q$ then exchange IC-signed versions of their supposedly common share, received from $\D$. Since a subset of {\it corrupt} parties
     belonging to $\Z_s$ {\it may not} respond and since the parties will {\it not} know the network type, the parties can only afford to wait till a subset of parties $\W_q \subseteq S_q$ have confirmed
     the receipt of a common share from $\D$, where $S_q \setminus \W_q \in \Z_s$ holds.
     Unfortunately, settling with a $\W_q$ where $S_q \setminus \W_q \in \Z_s$ {\it need not} guarantee that $\W_q$ has at least one {\it non-faulty} party, since $\W_q$ {\it need not} satisfy the
     $\Q^{(1)}(\W_q, \Z_s)$ condition. Also recall that as per semantics of linear secret-sharing with IC-signatures, we require the core-sets $\W_q$ to satisfy the condition $S_q \setminus \W_q \in \Z_a$, 
     {\it instead} of
      $S_q \setminus \W_q \in \Z_s$. 
      
      To deal with the above problem, we note that {\it irrespective} of the network type, there {\it always exist} a subset of parties $\specialS \in \ShareSpec_{\Z_s}$, 
      which consists of {\it only} non-faulty parties. And if $\D$ has distributed shares honestly, then the entire set of parties $\specialS$ will publicly report the pairwise consistency of their supposedly common share.
      Based on this observation, we now let $\D$ search for a candidate set $S_p$ from $\ShareSpec_{\Z_s}$ who have publicly confirmed the pairwise consistency of their supposedly common share.
      And once $\D$ finds such a candidate $S_p$, it computes and make public the core-sets $\W_q$ as per the following rules, for $q = 1, \ldots, |\Z_s|$.
      %----
      \begin{myitemize}
      %---
      \item[--] If the entire set of parties $S_q$ have confirmed the pairwise consistency of their supposedly common share, then set $\W_q = S_q$. \hfill {\bf (A)}
      %--
      \item[--] Else if $S_q \setminus (S_p \cap S_q) \in \Z_a$ {\it and} 
      the parties in $(S_p \cap S_q)$ have confirmed the consistency of their supposedly common share, then
      set  $\W_q = (S_p \cap S_q)$. \hfill {\bf (B)}
      %---
      \item[--] Else set $\W_q = S_q$ and make {\it public} the share $s_q$.  \hfill {\bf (C)}
      %---      
      \end{myitemize}
      %---
      The parties wait till they see $\D$ making public some set $S_p \in \ShareSpec_{\Z_s}$, along with sets $\W_1, \ldots, \W_{|\Z_s|}$. Upon receiving, the parties verify and ``approve" these sets
      as valid, provided the entire set of parties $S_p$ have confirmed the pairwise consistency of their supposedly common share and if each
      $\W_q$ is computed as per the rule {\bf (A), (B)} or {\bf (C)}. If $\W_1, \ldots, \W_{|\Z_s|}$ are approved then they indeed {\it satisfy} the requirements of core-sets as per our semantics of
      linear secret-sharing with IC-signatures. While this is trivially true if any $\W_q$ is computed either using rule {\bf (A)} or rule {\bf (B)}, the same holds even if 
      $\W_q$ is computed using rule {\bf (C)}. This is because in this case, the parties would publicly set $[s]_q = s_q$. Moreover, the parties would take the ``default" (linear) IC-signature of $s_q$ on the behalf of $S_q$,
      where the IC-signature as well as verification points are {\it all} set to $s_q$.
      
      Now let us analyze the above idea. If $\D$ is {\it non-faulty}, then {\it irrespective} of the network type, it will {\it always} find a candidate $S_p$ and hence compute and make public
      the core-sets $\W_1, \ldots, \W_{|\Z_s|}$ as per the above rules. This is because the set $\specialS$ consisting of {\it only} non-faulty parties {\it always} constitute a candidate $S_p$.
      Surprisingly and somewhat counter intuitively, we now show that even if the core-sets are computed with respect to some {\it different} candidate $S_p \neq \specialS$, a {\it non-faulty}
      $\D$ will {\it never} make public the share corresponding to $\specialS$, since the rule {\bf (C)} above will {\it not} be applicable over $\specialS$, 
      implying the privacy of $s$.
      If the network is {\it synchronous}, then the time at which $\D$ finds the set of parties in $S_p$ reporting 
      the pairwise consistency of their supposedly common share, will be the {\it same} at which the parties in $\specialS$ will report the pairwise consistency of their supposedly common share.
      This is ensured by maintaining sufficient ``timeouts" in the protocol to report pairwise consistency of supposedly common shares.
      Consequently, rule {\bf (A)} will be applied on $\specialS$.
      For an {\it asynchronous} network, rule {\bf (B)} will be {\it applicable} for $\specialS$, as
      $\specialS \setminus (S_p \cap \specialS) \in \Z_a$ will always hold.
      %--------       
     \subsubsection{Network Agnostic VSS for Multiple Dealers with Linearity}
     %---
     \paragraph{\bf Technical Challenge in $\VSS$ for Multiple Dealers.}
     %---
     While protocol $\VSS$ allows any {\it single} dealer to generate a $[\cdot]$-sharing of its input, we may ``loose" the linearity property offered by $[\cdot]$-sharing,
      if 
     {\it different} dealers invoke instances of $\VSS$ to secret-share their inputs, since the underlying core-sets might be {\it different} for different dealers.
     In more detail, let $\D_a$ and $\D_b$ be two {\it different} dealers with inputs $a$ and $b$ respectively, who invoke instances $\VSS^{(a)}$ and $\VSS^{(b)}$
     to generate $[a]$ and $[b]$ respectively. Let $\W_1^{(a)}, \ldots, \W_{|\Z_s|}^{(a)}$ and $\W_1^{(b)}, \ldots, \W_{|\Z_s|}^{(b)}$ be the underlying core-sets for 
          $\VSS^{(a)}$ and $\VSS^{(b)}$ respectively.  Now consider a scenario where for some $q \in \{1, \ldots, |\Z_s| \}$, the core-sets 
     $\W_q^{(a)}$ and $\W_q^{(b)}$ are different, even though both of them {\it satisfy} the condition $S_q \setminus \W_q^{(a)} \in \Z_a$
     and $S_q \setminus \W_q^{(b)} \in \Z_a$. Let $c \defined a + b$.
     Then the parties in $S_q$ can {\it non-interactively} compute their share $[c]_q$ corresponding to $[c]$ by setting $[c]_q = [a]_q + [b]_q$, where $[a]_q$ and $[b]_q$
     are the shares corresponding to $[a]$ and $[b]$ respectively, for the parties in $S_q$.
     We also note that as part of $[a]$, every (non-faulty) $P_i \in \W_q^{(a)}$ have the IC-signature $\{ \ICSig(P_j, P_i, P_k, [a]_q) \}_{P_j \in \W_q^{(a)}, P_k \not \in \W_q^{(a)}}$, while as part of
     $[b]$, every (non-faulty) $P_e \in \W_q^{(b)}$ have the IC-signature $\{ \ICSig(P_d, P_e, P_f, [b]_q) \}_{P_d \in \W_q^{(b)}, P_f \not \in \W_q^{(b)}}$, where the underlying IC-signatures satisfy the linearity property.
     However, since  $\W_q^{(a)} \neq \W_q^{(b)}$, it is {\it not} guaranteed that we have a core-set $\W_q^{(c)}$ as part of $[c]$, where $S_q \setminus \W_q^{(c)} \in \Z_a$, such that every
     (non-faulty) $P_i \in \W_q^{(c)}$ have the IC-signature $\{ \ICSig(P_j, P_i, P_k, [c]_q) \}_{P_j \in \W_q^{(c)}, P_k \not \in \W_q^{(c)}}$.
     Had it {\it been} the case that $\W_q^{(a)} = \W_q^{(b)}$, the parties could set $\W_q^{(c)}$ to $\W_q^{(a)}$ and the {\it linearity} of IC-signatures would have ensured that 
     every
     (non-faulty) $P_i \in \W_q^{(c)}$ {\it non-interactively} computes $\{ \ICSig(P_j, P_i, P_k, [c]_q) \}_{P_j \in \W_q^{(c)}, P_k \not \in \W_q^{(c)}}$ from
     the IC-signatures, held by $P_i$ as part of $[a]$ and $[b]$. In the {\it absence} of any set $\W_q^{(c)}$ with required IC-signatures, the {\it robust} reconstruction of the share $[c]_q$ 
     will {\it fail}, which further implies {\it failure} of shared circuit-evaluation of $\ckt$, where the inputs for $\ckt$ will be secret-shared by {\it different} parties.
     %----
     \paragraph{\bf Way Out.}
     %---
     To deal with the above problem, we ensure that the core-sets are {\it common} for {\it all} the secret-shared values during the circuit-evaluation. Namely, there exists {\it global} core-sets
     ${\GW}_1, \ldots, {\GW}_{|\Z_s|}$, where each ${\GW}_q$ satisfies the condition $S_q \setminus {\GW}_q \in \Z_a$, which constitute the core-sets for 
     {\it all} the secret-shared values during the circuit-evaluation. Note that maintaining a bunch of common core-sets across all the secret-shared values is extremely challenging in a network-agnostic setting,
     especially when the network is {\it asynchronous} and protocol $\VSS$ alone is {\it not sufficient} to achieve this goal. Rather we use a different approach. We generate a ``bunch" of linearly secret-shared
     random values with IC-signatures and common core-sets ${\GW}_1, \ldots, {\GW}_{|\Z_s|}$ in {\it advance} through another protocol called $\Rand$ (discussed in the next section).
     Later, if any party $P_i$ needs to secret-share some $x$, then one of these random values is reconstructed {\it only} towards $P_i$, who uses it as a one-time pad (OTP) and makes public an OTP-encryption of
     $x$. The parties can then take the ``default" secret-sharing of the OTP-encryption with IC-signatures and ${\GW}_1, \ldots, {\GW}_{|\Z_s|}$ as the core-sets and then non-interactively ``remove" the
     pad from the OTP-encryption by using the linearity property of secret-sharing, thus resulting in $[x]$, where the underlying core-sets are 
     ${\GW}_1, \ldots, {\GW}_{|\Z_s|}$. We call this protocol as $\LSh$.
          To ensure privacy of the values during the circuit-evaluation, we need to have $L$ number of secret-shared random values with 
     global core-sets being generated through $\Rand$, if $L$ is the maximum number of values which need to be secret-shared by different parties during the circuit-evaluation.
     We show that  $L \leq n^3 \cdot c_M + 4n^2 \cdot c_M + n^2 + n$ where $c_M$ is the number of multiplication gates in $\ckt$ 
     and consequently, $\Rand$ generates these many number of secret-shared random values with global core-sets.
     %----
     \subsubsection{Secret-Shared Random Values with Global Core Sets}
     \label{ssec:Rand}
     %---
     Protocol $\Rand$ allows the parties to generate linearly secret-shared random values with IC-signatures, where the underlying core-sets are {\it common} across all the secret-shared values.
     For simplicity, we explain the idea behind the protocol for generating one random value.
     The ``standard" way will be 
      to let each party $P_i$ pick a random value $r^{(i)}$ and generate $[r^{(i)}]$ by acting as a dealer and invoking an instance of $\VSS$.
     To avoid an endless wait, the parties can afford to only wait for the completion of $\VSS$ instances invoked by a set of parties $\PartySet \setminus Z$ for some $Z \in \Z_s$, even if the network is {\it synchronous}.
     This is because the corrupt dealers {\it may not} invoke their designated instances of $\VSS$. To find out
     the common subset of dealers whose $\VSS$ instances get completed for everyone, the parties run an instance of {\it agreement on a common subset} (ACS) primitive \cite{BKR94,CanettiThesis}, which involves
     invoking $n$ instances of our network agnostic BA, one on the behalf of each dealer, to decide the $\VSS$ instances of which dealers got over. Let $\C$ be the set of common dealers identified through 
     ACS, where $\PartySet \setminus \C \in \Z_s$. Due to the $\Q^{(2)}(\PartySet, \Z_s)$ condition, $\C$ is bound to have at least one {\it non-faulty} party who has shared a random value, unknown
     to the adversary.
     Hence, the sum of the values shared by all the dealers will be a random value for the adversary.
     %-------
     \paragraph{\bf Technical Challenges.}
     %---
     Even though the above approach is standard for generating a secret-shared random value, it {\it fails} in our context due to the following two ``problems" in the protocol $\VSS$.
     %---
      \begin{myitemize}
      %----
      \item[--] {\bf Problem I}: The first problem is that it {\it may not} be possible now to maintain the linearity of IC-signatures, across all the instances of $\VSS$.
      To understand the issue, consider a fixed triplet of parties, say $(P_i, P_j, P_k)$, where $P_i, P_j$ and $P_k$ are playing the role of $\S, \mathsf{I}$ and $\mathsf{R}$ respectively
      in the various instances of $\VSS$ invoked by different dealers.
      Now recall that to maintain the linearity of IC-signatures, it is {\it necessary} that $P_i$ selects the {\it same} set of supporting-verifiers
      $\R$ in {\it all} the underlying instances of  authentication phase involving $P_j$ and $P_k$.
      This is possible {\it only if} $P_i$ 
      knows {\it all} the values on which it wants to generate the IC-signature for $P_j$ 
      and $P_k$ and start invoking {\it all} the underlying instances of authentication phase.
      Instead, if $P_i$ starts invoking the instances of authentication phase {\it as and when} it has some data to be authenticated for $P_j$ and $P_k$,
      then it {\it may not} be possible that the set $\R$ is the {\it same} in all the ``past" and in the ``future" instances of authentication phase, involving $P_i, P_j$ and $P_k$ in the above roles, especially if the
      network is {\it asynchronous}. Since in $\VSS$, IC-signatures are generated on the supposedly common shares (after receiving them from the underlying dealer) 
      and since now multiple instances of $\VSS$ are invoked (by {\it different} dealers), 
       this means that $P_i$ should {\it first} have the data from all the dealers for the various instances of $\VSS$ and {\it then} start invoking instances of authentication phase to generate
       IC-signatures on these values for $P_j$.
       This is clearly {\it not} possible, especially if the network is {\it asynchronous}, since $P_i$ won't be knowing {\it beforehand} from which dealers it will be receiving shares as part of $\VSS$. \\[.2cm] 
      %----
      \noindent {\bf Way Out.} 
      %---
      To deal with the above issue, we now let the dealers publicly commit their shares as part of the $\VSS$ instances through a primitive called {\it secure verifiable multicast} (SVM).
      The primitive allows a designated {\it sender} $\Sender \in \PartySet$ with input $v$ to ``verifiably" send $v$ to a designated set of {\it receivers}  $\ReceiverSet \subseteq \PartySet$, such that if
      $\{\Sender \} \cup \ReceiverSet$ does not contain any corrupt party, then adversary {\it does not} learn any information about $v$.
      The verifiability here guarantees that even if $\Sender$ is {\it corrupt}, if the non-faulty
       parties in $\ReceiverSet$ get any value from $\Sender$, then it will be common and {\it all} the (non-faulty) parties in $\PartySet$ will be
        ``know" that $\Sender$ has sent some value to $\ReceiverSet$.
         Our instantiation of SVM is very simple: $\Sender$ acts as a dealer and generates $[v]$ by invoking an instance of $\VSS$. Once $[v]$ is generated, the parties in $\PartySet$ are aware
         that $\Sender$ is
        ``committed" to a value, which is not yet known. The next step is to let {\it only} the parties in $\ReceiverSet$ reconstruct $v$.
        
        Now using SVM, we let the various dealers to distribute the shares for their randomly chosen inputs (for $\Rand$)
         during the underlying instance of $\VSS$ as follows.
        Consider the dealer $P_{\ell}$ who has invoked an instance of $\VSS$ to secret-share a randomly chosen value $r^{(\ell)}$. For this, it picks 
        random shares
      $r^{(\ell)}_1, \ldots, r^{(\ell)}_{|\Z_s|}$ which sum up to $r^{(\ell)}$.
      Now instead of directly sending send $r^{(\ell)}_q$ to the parties in $S_q$, it invokes $|\Z_s|$ instances of SVM with input $r^{(\ell)}_1, \ldots, r^{(\ell)}_{|\Z_s|}$ and
      $S_1, \dots, S_{|\Z_s|}$ as the designated set of receivers respectively. 
      This serves {\it two} purposes. First, it is guaranteed that all the parties in $S_q$ receive a {\it common} share from $P_{\ell}$.
      Second and more importantly, {\it all} the parties in $\PartySet$ will now {\it know} that $P_{\ell}$ has distributed shares to each set from $\ShareSpec_{\Z_s}$.
     The parties then run an instance of ACS to identify a common subset of {\it committed dealers} $\CD \subseteq \PartySet$, where
      $\PartySet \setminus \CD \in \Z_s$, who have invoked the desired instances of SVM and delivered the required shares to each group $S_q \in \ShareSpec_{|\Z_s|}$. 
      The way timeouts are maintained as part of the ACS, it will be ensured that in a {\it synchronous} network, {\it all} {\it non-faulty} dealers are present in $\CD$.
      Once the set $\CD$ is identified, it is guaranteed that every {\it non-faulty} party $P_i$ will have the shares from {\it all} the dealers in $\CD$. And once it has the shares from all the dealers in $\CD$, it starts
      generating the IC-signatures on these shares for the designated parties as part of the $\VSS$ instances corresponding to the dealers in $\CD$ and ensures that all the pre-requisites are satisfied
      to guarantee the linearity of the underlying IC-signatures.
      Now {\it instead} of selecting the set of dealers $\C$ (for $\Rand$) from $\PartySet$, the parties run an instance of ACS over the set of committed dealers $\CD$ to
       select $\C$ where $\CD \setminus \C \in \Z_s$ holds.
       
       We stress that we now need {\it two} instances of ACS during $\Rand$, the first instance is required to identify the set of committed dealers $\CD$ who have distributed shares,
        while the second instance is required to identify the set of committed dealers 
       $\C$, whose underlying instance of $\VSS$ will complete for everyone. We also stress that {\it irrespective} of the network type, the set $\C$ is still now guaranteed to have at least one non-faulty party.
       While this is trivially true in an {\it asynchronous} network where $\Z_a$ satisfies the $\Q^{(1)}(\C, \Z_a)$ condition, the same is true in the {\it synchronous} network because 
       $\CD$ will have {\it all} non-faulty dealers and hence $\Z_s$ will satisfy the $\Q^{(1)}(\C, \Z_s)$ condition.      
            %---
      \item[--] {\bf Problem II}:
      %---
      Even if we apply the idea of first finding the set of committed dealers $\CD$, we {\it still} have the following problem in protocol $\Rand$: it is {\it not} ensured that
      the underlying core-sets are {\it common} for the values shared by the dealers in the set $\C$. Namely, it might be possible that $P_i \in \C$ and has generated $[r^{(i)}]$ with 
      $\W^{(i)}_1, \ldots, \W^{(i)}_{|\Z_s|}$ as the core-sets, while there exists another dealer $P_j \in \C$ who has generated 
       $[r^{(j)}]$ with 
      $\W^{(j)}_1, \ldots, \W^{(j)}_{|\Z_s|}$ as the core-sets, such that there exists some $q \in \{1, \ldots, |\Z_s| \}$ where 
      $\W^{(i)}_q \neq \W^{(j)}_q$.
      Instead we require every dealer in $\CD$ (and hence $\C$) to secret-share their corresponding random values in such a way that the underlying core-sets are common. Only then it will be ensured that the random values
      generated through $\Rand$ (obtained by summing up the values shared by the different dealers in $\C$) are secret-shared with common core-sets. \\[.2cm]
      %---
      \noindent{\bf Way Out.} Getting rid of the above problem is {\it not} possible if we let every dealer in $\CD$ to compute {\it individual} core-sets during their respective instances of $\VSS$, as per the steps of
      $\VSS$. Recall that in $\VSS$, the dealer $\D$ computes the underlying core-sets with respect to the ``first" set $S_p$ from $\ShareSpec_{|\Z_s|}$ such that the parties in $S_p$ have confirmed
      the pairwise consistency of their supposedly common share after exchanging IC-signatures on these values.
      As a result, it might be possible that there is some dealer $\D \in \CD$ who computes the core-sets in its instance of $\VSS$ with respect to $S_p \in \ShareSpec_{\Z_s}$, while
      there exists {\it another} dealer $\D' \in \CD$  who computes the core-sets in its instance of $\VSS$ with respect to $S'_p \in \ShareSpec_{\Z_s}$ where
      $S_p \neq S'_p$, thus resulting in {\it different} core-sets in the corresponding $\VSS$ instances.
      
      To deal with the above issue, we {\it instead} let each dealer in $\CD$ to {\it continue} computing and publishing {\it different} core-sets with respect to various ``eligible" candidate 
      $S_p$ sets from $\ShareSpec_{\Z_s}$  and let the parties run an instance of ACS to identify a {\it common} subset of dealers $\C \in \CD$ where $\CD \setminus \C \in \Z_s$, such that {\it all} the dealers
      have computed and published ``valid" core-sets, computed with the respect to the {\it same} $S_p \in \ShareSpec_{\Z_s}$.
      The idea here is that there always exists a set $\specialS \in \ShareSpec_{\Z_s}$ consisting of {\it only} non-faulty parties ({\it irrespective} of the network type).
      So if the dealers in $\CD$ keep computing and publishing {\it all possible} candidate core-sets  in their respective $\VSS$ instances, then the set of {\it non-faulty} dealers $\Hon$ in $\CD$
      will compute and publish core-sets with respect to $\specialS$ ({\it irrespective} of the network type). This is because the parties in $\specialS$ will indeed publicly confirm the pairwise consistency
      of their supposedly common share and exchange IC-signatures in the $\VSS$ instances of {\it all} the dealers in $\Hon$.
      Hence $\Hon$ and $\specialS$ {\it always} constitute the candidate $\CD$ and the common $S_p$ set that we are looking for. 
      
      Note that identifying $\C$ out of $\CD$ through ACS is {\it non-trivial} and requires carefully executing
      the underlying instances of (network agnostic) BA, invoked as part of ACS.
      In fact we run the BA instances in  ``two-dimensions".
      We first run $|\Z_s|$ instances of $\BA$, one on the behalf of each set in $\ShareSpec_{\Z_s}$, where the $q^{th}$ instance is executed to decide whether a subset of dealers in $\CD \setminus Z$ for some
      $Z \in \Z_s$
      have published valid core-sets with respect to the set $S_q \in \ShareSpec_{\Z_s}$.
      This enables the parties to identify a {\it common} set $S_{\qcore} \in \ShareSpec_{\Z_s}$, such that it is guaranteed that a subset of 
      dealers in $\CD \setminus Z$ for some
      $Z \in \Z_s$
      have indeed published valid core-sets with respect to the set $S_{\qcore}$.
      Once the set $S_{\qcore}$ is identified, the parties then run $|\CD|$ instances of BA to decide which dealers in $\CD$ have 
      published core-sets with respect to $S_{\qcore}$.
      %-----
      \end{myitemize}
     %----     
     \subsubsection{Network Agnostic Secure Multiplication}
     \label{ssec:Mult}
     %---
     The key subprotocol behind our multiplication protocol is a {\it non-robust} multiplication protocol $\BasicMult$ (standing for basic multiplication), which takes input 
        $[a]$ and $[b]$ and an {\it existing} set of {\it globally discarded} parties $\Discarded$, which contains only {\it corrupt} parties.
       The protocol securely generates $[c]$  {\it without}
      revealing any additional  information about $a, b$ (and $c$). 
       If {\it no} party in $\PartySet \setminus \Discarded$ cheats, then $c = a \cdot b$ holds.
       The idea behind the protocol is to let each {\it summand} $[a]_p \cdot [b]_q$ being secret-shared by a {\it summand-sharing party}. Then $[a \cdot b]$ can be computed
       using the linearity of secret-sharing and the fact that the following holds:
       %----
       \[ [a \cdot b] =   \displaystyle \sum_{(p, q) \in \{1, \ldots, |\Z_s| \} \times \{1, \ldots, |\Z_s| \}} [[a]_p \cdot [b]_q].\]
       %---
      Existing multiplication protocols in the {\it synchronous} and {\it asynchronous} setting \cite{HT13,ACC22c} also use an 
      instantiation of $\BasicMult$, based on the above idea. 
      In the sequel, we briefly recall them, followed by the technical challenges faced in the network agnostic setting and how we deal with them
      counter-intuitively.
      %----
      \paragraph{\bf $\BasicMult$ in the Synchronous Setting with $\Q^{(2)}(\PartySet, \Z_s)$ Condition \cite{HT13}.}
      %---
      In \cite{HT13}, each summand $[a]_p \cdot [b]_q$ is {\it statically} assigned to a {\it designated} summand-sharing party for secret-sharing through some publicly known deterministic summand assignment,
       which is possible since
      $[a]_p$ and $[b]_q$ are held by the parties in $S_p \in \ShareSpec_{\Z_s}$ and $S_q \in \ShareSpec_{\Z_S}$ respectively and $(S_p \cap S_q) \neq \emptyset$, if
      $\Q^{(2)}(\PartySet, \Z_s)$ condition holds.
      Hence the set of parties $(S_p \cap S_q)$ who can compute and secret-share the summand $[a]_p \cdot [b]_p$ is {\it non-empty}.
           Since the parties in $\Discarded$ are {\it already} known to be corrupted, all the shares $[a]_p$ and $[b]_q$ held by the parties in $\Discarded$
      are {\it publicly reconstructed} and {\it instead} of letting the parties in $\Discarded$ to secret-share the assigned summands, the parties take the ``default" secret-sharing
      of the summands ``assigned" to the parties in $\Discarded$. This {\it prevents} the already known corrupt parties to again cheat by secret-sharing an incorrect summand. 
      It is easy to see that if {\it none} of the parties in $\PartySet \setminus \Discarded$ cheats, then the parties output $[a \cdot b]$.
       %----      
        \paragraph{\bf $\BasicMult$ in the Asynchronous Setting with $\Q^{(3)}(\PartySet, \Z_a)$ Condition \cite{ACC22c}.}
       %---
       The idea of {\it statically} designating each summand $[a]_p \cdot [b]_q$ to a {\it unique} party in $\PartySet \setminus \Discarded$
        {\it need not} work in the {\it asynchronous} setting, since the designated party may be {\it corrupt} and need not secret-shared any summand, thus resulting in an {\it endless} wait.
        To deal with this challenge, \cite{ACC22c} {\it dynamically} selects the summand-sharing parties for each summand.
        In more detail, let 
        $\Z_a = \{\mathsf{Z}_1, \ldots, \mathsf{Z}_{|\Z_a|} \}$ and $\ShareSpec_{\Z_a} = \{\S_1, \ldots, \S_{|\Z_a|} \}$, where each $\S_r = \PartySet \setminus \mathsf{Z}_r$
        Now since the $\Q^{(3)}(\PartySet, \Z_a)$ condition is satisfied and $\Discarded \in \Z_a$, it follows that $(\S_p \cap \S_q) \setminus \Discarded \neq \emptyset$.
        This implies that there exists at least one non-faulty party in $(\S_p \cap \S_q)$ who has both the share $[a]_p$ as well as $[b]_q$ and hence can secret-share
        the summand $[a]_p \cdot [b]_q$. Hence {\it every} party in $\PartySet \setminus \Discarded$ is allowed to secret-share {\it all} the summands it is ``capable" of, with a special care taken to ensure
        that each summand $[a]_p \cdot [b]_q$ is considered {\it exactly once}.
        To ensure this, the protocol now proceeds in ``hops", where in each hop all the parties in $\PartySet \setminus \Discarded$ secret-share all the summands they are capable of, {\it but} a {\it single}
        summand sharing party is finally selected for the hop through ACS. Then to {\it avoid} repetition, all the summands which have been shared by the most recently elected summand-sharing party
        are ``marked" as shared and not considered for sharing in the future hops by any future summand-sharing party. Moreover, a party who has already served as a summand-sharing party is {\it not}
        allowed to again get selected as a summand-sharing party in the future hops.
        %----        
       \paragraph{\bf Technical Challenges in the Network Agnostic Setting.}
       %--- 
       From the above discussion it follows that in the network agnostic setting, 
        the {\it asynchronous} $\BasicMult$ based on {\it dynamically} selecting summand-sharing parties
         will {\it fail} if the network turns out to be {\it synchronous}, since $\Q^{(3)}$ condition {\it need not} be satisfied.
       On the {\it synchronous} $\BasicMult$ based on {\it statically} selecting summand-sharing parties will {\it fail} if a designated summand-sharing party {\it does not} secret-shares the required summands,
       resulting in an endless wait, since the parties will {\it not} be knowing the network type.
       The way out is to select summand-sharing parties in {\it three} phases. We 
       {\it first} select summand-sharing parties dynamically in {\it hops}, following the approach of \cite{ACC22c}, till we find any subset of parties from $\ShareSpec_{\Z_s}$,
        who have shared {\it all} the summands 
       they are capable of. Then in the {\it second} phase, the {\it remaining} summands which are {\it not} yet secret-shared are {\it statically} assigned and the respective designated summand-sharing
       parties are asked to secret-share the assigned summands. 
       As the corrupt parties {\it may not} share the assigned summands during this phase, the parties wait only for a ``fixed" time required for the parties to secret-share the assigned summands in a {\it synchronous}
       network and then run instances of BA to identify which of the designated summand-sharing parties have turned up during the second phase.
       Finally, during the {\it third} phase, any ``leftover" summands which are {\it not yet} shared during either phase is {\it publicly} reconstructed by reconstructing the
       corresponding shares and a default sharing is taken for such summands.
     
       
       The idea here is the following: {\it all} non-faulty parties will 
        share all the summands, which are assigned to them, either statically or dynamically, {\it irrespective} of the network type.
        Consequently, the first phase will be always over, since the set consisting of {\it only} non-faulty parties always constitute the candidate
        set of summand-sharing parties, which the parties are looking for the completion of the first phase.
        Once the first phase is over, the second phase is bound to be over since there we wait {\it only} for a fixed time.
        The third phase is always bound to be over, once the first two phases are over, since it involves publicly reconstructing only the leftover summands.
        The way summands are assigned across the three phase, it will be always guaranteed that every summand is considered for sharing once in exactly one of the three phases and no summand will be left out,
        since in the worst case, we always have the {\it third} phase, where any leftover summand is publicly reconstructed. The crucial point here is that the 
        the shares held {\it only} by the non-faulty parties {\it never} get publicly reconstructed, thus guaranteeing that the adversary {\it does not} learn any additional information about $a$ and $b$. 
        This is obviously true in a {\it synchronous} network because in the ``worst" case, we always have the {\it second} phase where every non-faulty party 
         who is {\it not} selected as a summand-sharing party in any of the hops during the first phase 
        will get the opportunity
        to secret-share their assigned summands. 
        On the other hand, in an {\it asynchronous} network, it can be shown that {\it all} the summands which involve any share held by the non-faulty parties would have been secret-shared  
        during the {\it first} phase itself. In more detail, let $Z^{\star} \in \Z_a$ be the set of {\it corrupt} parties and let $\Hon = \PartySet \setminus Z^{\star}$ be the set of {\it honest} parties. 
        Moreover, let $S_h \in \ShareSpec_{\Z_s}$ be the group consisting of {\it only} honest parties; i.e. $(S_h \cap Z^{\star}) = \emptyset$.
       The parties in $S_h$ hold the shares $[a]_h$ and $[b]_h$.
        Now consider an {\it arbitrary} summand $[a]_h \cdot [b]_q$. Suppose the first phase gets over because it is found that every party in $S_{\ell} \in \ShareSpec_{\Z_s}$
        has been selected as a summand-sharing party in some hop during the {\it first} phase.         
        Then consider the set $(\Hon \cap S_{\ell} \cap S_q)$, which is {\it not} empty, if 
       the $\Q^{(2, 1)}(\PartySet, \Z_s, \Z_a)$ condition is satisfied. 
       Hence there exists {\it some} 
      $P_j \in (\Hon \cap S_{\ell} \cap S_q)$,
      who would have shared the summand $[a]_h \cdot [b]_q$ when selected as a summand-sharing party during some hop in the first phase. 
      Due to a similar reason, any summand of the form $[a]_q \cdot [b]_h$ would have been secret-shared during the first phase itself. 
      %---             
     \subsection{Other Related Works}
     %---
     The domain of network agnostic cryptographic protocols is relatively new and almost all the existing works have considered {\it threshold} adversaries. 
       The work of  \cite{BKL21} presents a network agnostic {\it cryptographically-secure} atomic broadcast protocol. 
     The work of \cite{MO21} studies 
     Byzantine fault tolerance and state machine replication protocols for multiple thresholds, including $t_s$ and $t_a$. 
     The work of \cite{GLW22} presents a network agnostic protocol for the task of approximate agreement using the condition
     $2t_s + t_a < n$. The same condition has been used to design a network agnostic distributed key-generation (DKG) protocol in \cite{BCLL22}. 
           A recent work \cite{DL22} has studied the problem of network agnostic perfectly-secure message transmission (PSMT) \cite{DDWY93} over {\it incomplete} graphs.
     %---------     
     \subsection{Open Problems}
     %---------
     There are several interesting directions to explore for network agnostic MPC protocols. Here we mention few of them.
     It is {\it not} known whether the conditions $3t_s + t_a < n$ (resp.~$\Q^{(3, 1)}(\PartySet, \Z_s, \Z_a)$)
     is {\it necessary} for the network agnostic MPC with {\it perfect} security against threshold (resp.~non-threshold) adversary.
     An abundant amount of research effort has been spent to improve both the theoretical as well as practical efficiency of (unconditionally-secure) SMPC and AMPC protocols.
     The works of \cite{ACC22a,ACC22b} and this work just focus on the {\it possibility} of unconditionally-secure network agnostic MPC. 
     Upgrading the efficiency of these protocols and making it closer to that of SMPC and AMPC protocols seem to require a significant research effort.
     Even though the complexity of our MPC protocol is polynomial in $n$ and $|\Z_s|$, when instantiated for {\it threshold} adversaries (where $|\Z_s|$ has all subsets of $\PartySet$ of size up to $t_s$)
     may result in {\it exponential} (in $n$) amount of computation and communication. This is {\it unlike} the case for {\it perfect security}, where we have network agnostic MPC 
     protocol against threshold adversaries
     with polynomial (in $n$) complexity \cite{ACC22a}. Hence designing network agnostic MPC protocol against {\it threshold} adversaries with {\it statistical} security and {\it polynomial} complexity is left as a challenging open 
     problem.     
     %%%%%%%%%%%%OLD STUFF%%%%%%%
     \begin{comment}
     %---
         However, {\it non-repudiation} is {\it not} guaranteed in a {\it synchronous} network, since a potentially {\it corrupt} $\S$ may {\it not} include {\it all} the honest verifiers
       in $\R$. Consequently, the verification-point of {\it all corrupt} verifiers in $\R$ may end up being {\it not} accepted, while the accepted
       verification-points, revealed by the {\it honest} verifiers
       in $\R$ {\it may not} be in ``sufficient number" to accept the revealed $F(x)$. To deal with this, we now {\it additionally} check, if the verification-points which are {\it not} accepted 
       (at an appropriate time), correspond to a set of parties $\R''$ where $\R'' \in \Z_s$. And if so, then $\Receiver$ still accepts $F(x)$, if it finds a candidate $\R'$.  
        The protocol is presented in Fig \ref{fig:ICP}, where all instances of broadcast happen through protocol $\BC$.

     
     %---
     \end{comment}
     

       

==> symbols_env.tex <==
%--------------------------------------------------------------
%New Style boxes
%--------------------------------------------------------------



%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}

%Basic box structure with title box
\newenvironment{titlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		%skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		%skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=15pt}\setlist[enumerate]{leftmargin=15pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonbox}{%
	%align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	%innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	%splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}


\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gsystembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}
	
	

\newenvironment{protocolbox}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}


\newenvironment{algobox}[3]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{reductionbox}[3]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gamebox}[3]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
%Split Box for IEETran Version
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{splittitlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\mdfdefinestyle{commonsplitbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}

\newenvironment{protocolsplitbox}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
\newenvironment{schemesplitbox}[3]
{\begin{splittitlebox}{Functionality \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
	
\newenvironment{simulatorsplitbox}[3]
{\begin{splittitlebox}{Simulator \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}	
	
\newenvironment{experimentsplitbox}[3]
{\begin{splittitlebox}{Experiment \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}	


%------------------------------------------------------------------------------
% Full Width Environments
%------------------------------------------------------------------------------

\newenvironment{systembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gsystembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{protocolbox*}[3]
{\begin{strip}
\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{algobox*}[3]
{\begin{strip}
\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{reductionbox*}[3]
{\begin{strip}
\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gamebox*}[3]
{\begin{strip}
\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{simulatorbox*}[3]
{\begin{strip}
\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}




%------------------------------------------------------------------------------
%Basic box structure with mytitle box without embossed title
%------------------------------------------------------------------------------

%box style
\mdfdefinestyle{mycommonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=3pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
}
\mdfdefinestyle{myroundbox}{style=mycommonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{titlebox*}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=0.3\baselineskip,
		skipabove={0.4em},
		skipbelow={1em},needspace=3\baselineskip,
		frametitleaboveskip=5em,
		innerrightmargin=5pt
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\normalfont \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%------------------------------------------------------------------------------
% Box Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox}[3]
{\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygsystembox}[3]
{\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myprotocolbox}[3]
{\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myalgobox}[3]
{\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myreductionbox}[3]
{\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygamebox}[3]
{\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mysimulatorbox}[3]
{\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}
%-------------------------------------------------------------------------------


%------------------------------------------------------------------------------
% Full Width Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygsystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myprotocolbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myalgobox*}[3]
{\begin{strip}
		\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myreductionbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygamebox*}[3]
{\begin{strip}
		\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mysimulatorbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}






%-------------------------------------------------------------------------------
% Basic protocol box without Algohead NDSS
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{mytbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mytsplitbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.8em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mypbox}[3]
{\begin{mytbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytbox}}

\newenvironment{mypsplitbox}[3]
{\begin{mytsplitbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytsplitbox}}












